Insights from GitHub Community on the Matter Standard: Developer Perspectives and Challenges

Matter seeks to resolve longstanding interoperability problems in the Internet of Things (IoT), yet little is known about how developers experience the standard in day to day work. This paper examines over 13,000 issues from the official Project CHIP GitHub repository to understand the kinds of problems contributors report when implementing and integrating Matter. Using topic modeling and qualitative analysis, we identify four recurring areas of concern, Testing, Interoperability, Development, and Platform and Network, and describe how they manifest in the evolution of the codebase and tooling. The findings reveal systematic technical and integration challenges and point to concrete opportunities to refine Matter's test infrastructure, cross vendor guidance, and documentation as the standard continues to mature.

==> visuals/broad_categories_count.tex <==
% \begin{table}[ht]
%     \centering
%     \caption{Broad Categories of Issues}
%     \begin{tabular}{@{}lll@{}}
%         \toprule
%         \textbf{Broad Category} & \textbf{Issue Count} & \textbf{Percentage} \\ \midrule
%         Testing                  & 5545                 & 42.63\%             \\
%         Interoperability         & 3926                 & 30.18\%             \\
%         Development              & 2087                 & 16.04\%             \\
%         Platform \& Network      & 1450                 & 11.15\%             \\ 
%         \bottomrule
%     \end{tabular}
%     \label{tab:issue_categories}
% \end{table}

==> visuals/topics_table.tex <==
% \begin{table*}[] % Use "table*" for two-column tables
%     \centering
%     \setlength\extrarowheight{3.5pt}
%     \label{visual:topics_table}
%     \title{Topics \& Keywords}
%     \caption{Topic number along with the labels, category, and top keywords for generated Matter GitHub Issues.}
%     \resizebox{\textwidth}{!}{ % Resize the table to fit the text width
%     \begin{tabular}{@{\extracolsep{5pt}}l l l l@{}}
%         \toprule
%         \textbf{Topic Number} & \textbf{Keywords} & \textbf{Label} & \textbf{Category} \\
%         \midrule
%         0 & chip, info, file, python, lib, line, src, connectedhomeip, test, stdout & Matter Build \& Integration & Development \\
%         1 & thread, wifi, ble, matter, network, commissioning, nxp, silabs, platform, support & Network \& Platform Setup & Platform \& Network \\
%         2 & build, matter, include, darwin, linux, building, arm, readable, file, export & Build Systems & Development \\
%         3 & test, tc, chip, spec, connectedhomeip, cluster, specifications, xml, attribute, python & Specification Testing & Testing \\
%         4 & dl, type, dmg, ota, msg, key, em, command, dis, received & Connectivity & Platform \& Network \\
%         5 & app, cluster, clusters, chip, server, cpp, attributes, attribute, data, connectedhomeip & Cluster Management & Development \\
%         6 & class, testing, support, unit, tests, function, implementation, api, data, functions & Hardware-based Security & Testing \\
%         7 & testing, tests, fix, changes, files, test, fixes, zap, summary, unit & Testing Maintenance & Testing \\
%         8 & chip, tool, log, dmg, command, dut, tc, error, test, user & Testing Tools & Testing \\
%         9 & third, party, pigweed, lwip, source, pw, file, python, src, target & Dependency and Environment Configuration & Interoperability \\
%         10 & request, guidelines, pydata, actions, sphinx, theme, formatting, force, readability, apply & Documentation Maintenance & Development \\
%         11 & app, esp, android, tv, camera, linux, casting, using, controller, webrtc & Application Interface & Interoperability \\
%         12 & platform, response, version, sdk, bug, reproduction, hash, prevalence, tested, type & Cross Platform & Interoperability \\
%         13 & openthread, details, summary, close, reopen, merge, br, redirect, upgrade, creating & Third-Party Dependency & Platform \& Network \\
%         14 & test, coding, cluster, problem, location, endpoint, spec, conformance, name, rule & Cluster and Testing Conformance & Testing \\
%         15 & device, icd, fabric, check, discussion, connectedhomeip, apple, subscription, chip, value & Fabric State Management & Interoperability \\
%         16 & connectedhomeip, chip, doc, update, title, testing, size, docker, see, increase & Docker Build Environment & Development \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table*}


\begin{table*}[ht] % Use regular table for better control
    \centering
    \setlength\extrarowheight{3.5pt} % Optional: adjust row height
    \title{Topics \& Keywords}
    \caption{Topic numbers along with labels and categories for generated Matter GitHub Issues.}
    \label{visual:topics_table}
    \resizebox{\textwidth}{!}{ 
    \begin{tabular}{@{\extracolsep{5pt}}l l l l@{}}
        \toprule
        \textbf{Topic\#} & \textbf{Keywords} & \textbf{Label} & \textbf{Category} \\
        \midrule
        0 & chip, info, file, python, lib, line, src, connectedhomeip, test, stdout & Matter Build \& Integration & Development \\
        1 & thread, wifi, ble, matter, network, commissioning, nxp, silabs, platform, support & Network \& Platform Setup & Platform \& Network \\
        2 & build, matter, include, darwin, linux, building, arm, readable, file, export & Build Systems & Development \\
        3 & test, tc, chip, spec, connectedhomeip, cluster, specifications, xml, attribute, python & Specification Testing & Testing \\
        4 & dl, type, dmg, ota, msg, key, em, command, dis, received & Connectivity & Platform \& Network \\
        5 & app, cluster, clusters, chip, server, cpp, attributes, attribute, data, connectedhomeip & Cluster Management & Development \\
        6 & class, testing, support, unit, tests, function, implementation, api, data, functions & Hardware-based Security & Testing \\
        7 & testing, tests, fix, changes, files, test, fixes, zap, summary, unit & Testing Maintenance & Testing \\
        8 & chip, tool, log, dmg, command, dut, tc, error, test, user & Testing Tools & Testing \\
        9 & third, party, pigweed, lwip, source, pw, file, python, src, target & Dependency and Environment Configuration & Interoperability \\
        10 & request, guidelines, pydata, actions, sphinx, theme, formatting, force, readability, apply & Documentation Maintenance & Development \\
        11 & app, esp, android, tv, camera, linux, casting, using, controller, webrtc & Application Interface & Interoperability \\
        12 & platform, response, version, sdk, bug, reproduction, hash, prevalence, tested, type & Cross Platform & Interoperability \\
        13 & openthread, details, summary, close, reopen, merge, br, redirect, upgrade, creating & Third-Party Dependency & Platform \& Network \\
        14 & test, coding, cluster, problem, location, endpoint, spec, conformance, name, rule & Cluster and Testing Conformance & Testing \\
        15 & device, icd, fabric, check, discussion, connectedhomeip, apple, subscription, chip, value & Fabric State Management & Interoperability \\
        16 & connectedhomeip, chip, doc, update, title, testing, size, docker, see, increase & Docker Build Environment & Development \\
        \bottomrule
    \end{tabular}
    }
\end{table*}

==> visuals/user_assigned_labels.tex <==
% \begin{table}[t]
%     \centering
%     \caption{Popular User Labels Issue and Their Counts}
%     \begin{tabular}{@{}ll@{}}
%         \toprule
%         \textbf{Category} & \textbf{Count} \\ \midrule
%         review - approved & 4708 \\
%         review - pending  & 3126 \\
%         examples          & 2930 \\
%         app               & 2427 \\
%         needs triage      & 2168 \\
%         fast track        & 2104 \\
%         tests             & 1965 \\
%         platform          & 1859 \\
%         darwin            & 1771 \\
%         bug               & 1500 \\
%         scripts           & 1363 \\
%         controller        & 1271 \\
%         github            & 1033 \\ 
%         \bottomrule
%     \end{tabular}
%     \label{tab:user_labels}
% \end{table}
